Foundations of Modern Query Languages for Graph Databases

We survey foundational features underlying modern graph query languages. We first discuss two popular graph data models: edge-labelled graphs, where nodes are connected by directed, labelled edges; and property graphs, where nodes and edges can further have attributes. Next we discuss the two most fundamental graph querying functionalities: graph patterns and navigational expressions. We start with graph patterns, in which a graph-structured query is matched against the data. Thereafter we discuss navigational expressions, in which patterns can be matched recursively against the graph to navigate paths of arbitrary length; we give an overview of what kinds of expressions have been proposed, and how they can be combined with graph patterns. We also discuss several semantics under which queries using the previous features can be evaluated, what effects the selection of features and semantics has on complexity, and offer examples of such features in three modern languages that are used to query graphs: SPARQL, Cypher and Gremlin. We conclude by discussing the importance of formalisation for graph query languages; a summary of what is known about SPARQL, Cypher and Gremlin in terms of expressivity and complexity; and an outline of possible future directions for the area.

==> type.tex <==
\section{Type Modifiers} \label{type} 

%\begin{itemize}
%\item Ungroup paths
%\item Obtain labels or attribute values
%\item Construct new graphs 
%\item Order by
%\item Limit
%\item What else?
%\end{itemize}


\subsection{Graph Transformations}

Until now, we have concentrated our interest on the issues related to querying graph data.
However, it is natural that the user requires not only to query the data, but also to integrate, filter and transform them.
The notion of data transformation have been largely used in databases, in particular in data fromousing, where the process of data integration is referred as ETL, i.e. extract, transform and load.
Here, data transformation implies to convert the extracted data from its previous form into the form needed to be stored and analyzed. 
Specifically, data transformation occurs by using rules or lookup queries or by combining the data with other data.

%Hence, we will use the term \emph{data extraction} as the process of retrieving and transforming the data from the database for further data processing (e.g. data analysis) or data storage (e.g. data migration).

Currently, data transformation is used in multiple application domains. 
 For instance, in social network analysis it is common to build a ``smaller' network based on relevant pieces of the huge network.
 This ``summarization'' is achieved by querying the data and applying transformation operations, e.g. to convert attributes into actors, to aggregate data of actors into attributes, or to generate complex relationships (having arity greater than two) from simple (binary) relationships \cite{90697}.
 Next we present an example of such transformations.        
 
\begin{example}
Let $G$ be the social network graph presented in Figure \ref{fig:sn-sample}.
The most simple type of transformation is a traditional query that extracts data from the database. 
 For instance, Figure \ref{fig:transf1} shows a subgraph obtained by filtering nodes labelled \emph{person} in $G$. 
 On the other hand, a powerful feature of a data transformation language is its ability to create new data.
 For instance, the graph in Figure \ref{fig:transf1} can be transformed into the graph in Figure \ref{fig:transf2} where the attribute \emph{country} has been transformed into a node \emph{Country} which is accompanied with two new edges labelled \emph{livesIn}.
 Finally, a transformation can use an aggregate operator in order to produce a ``summary graph''. For instance, the graph in Figure \ref{fig:transf3} summarizes the graph in Figure \ref{fig:transf2} by counting the number of outgoing edges of the node \emph{Country} and storing the result as the value of the new property \emph{inhabitants}.  
\end{example}

 
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}

%%%%% node n1 
\node[rect] (n1) {
\alt{64pt}{
\uri{firstName =} & \uri{``Julie"}\\
\uri{lastName =} & \uri{``Freud"}\\
\uri{country =} & \uri{``Chile"}
}};

%%%%% label of n1
\node[rt] (ln1) at (n1.north) {\uri{$n_1$ $:$ Person}};

%%%%% node n2
\node[rect, right=3cm of n1] (n2) {
\alt{60pt}{ 
\uri{firstName =} & \uri{``John"}\\
\uri{lastName =} & \uri{``Cook"}\\
\uri{country =} & \uri{``Chile"}
}};

%%%%% label of n2
\node[rt] (ln2) at (n2.north) {\uri{$n_2$ $:$ Person}};

%%%%% edge e1
\draw[arrout,bend left=10] (n1) to 
node[below, rectw] (e1) {} 
(n2);

%%%%% label of e1
\node[rt] (le1) at (e1.north) {\uri{$e_1$ $:$ knows}};

%%%%% edge e2
\draw[arrout,bend left=10] (n2) to 
node[below, rectw] (e2) {} 
(n1);

%%%%% label of e2
\node[rt] (le2) at (e2.north) {\uri{$e_2$ $:$ knows}};

\end{tikzpicture}
\end{center}
\caption{
Example of transformation 1. 
From the graph in Figure \ref{fig:sn-sample}, we have applied a simple
selection (filtering) of nodes to those labelled \emph{Person}.
\label{fig:transf1}}
\end{figure} 
 
%-----------------------------------------------------
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}

%%%%% node n1 
\node[rect] (n1) {
\alt{64pt}{
\uri{firstName =} & \uri{``Julie"}\\
\uri{lastName =} & \uri{``Freud"}
}};

%%%%% label of n1
\node[rt] (ln1) at (n1.north) {\uri{$n_1$ $:$ Person}};

%%%%% node n2
\node[rect, right=9cm of n1] (n2) {
\alt{60pt}{ 
\uri{firstName =} & \uri{``John"}\\
\uri{lastName =} & \uri{``Cook"}
}};

%%%%% label of n2
\node[rt] (ln2) at (n2.north) {\uri{$n_2$ $:$ Person}};

%%%%% node n6 
\node[rect,right=3cm of n1] (n6) {
\alt{71pt}{ 
\uri{name =} & \uri{``Chile"}
}};

%%%%% label of n6
\node[rt] (ln6) at (n6.north) {\uri{$n_6$ $:$ Country}} ;

%%%%% edge e8
\draw[arrout] (n1) to
node[below, rectw] (e8) {}
(n6);

%%%%% label of e8
\node[rt] (le8) at (e8.north) {\uri{$e_8$ $:$ livesIn}};

%%%%% edge e9
\draw[arrout] (n2) to
node[below, rectw] (e9) {}
(n6);

%%%%% label of e9
\node[rt] (le9) at (e9.north) {\uri{$e_9$ $:$ livesIn}};

\end{tikzpicture}
\end{center}
\caption{Example of transformation 2.
Using the graph in Figure \ref{fig:transf1}, the \emph{country} attribute (of the nodes \emph{Person}) has been transformed into a node \emph{Country} including the attribute \emph{name}.} 
\label{fig:transf2}
\end{figure} 


%-----------------------------------------------------
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}

%%%%% node n6 
\node[rect,right=3cm of n1] (n6) {
\alt{71pt}{ 
\uri{name =} & \uri{``Chile"}\\
\uri{inhabitants =} & \uri{``2"}
}};

%%%%% label of n6
\node[rt] (ln6) at (n6.north) {\uri{$n_6$ $:$ Country}} ;

\end{tikzpicture}
\end{center}
\caption{Example of transformation 3. 
Given the graph in Figure \ref{fig:transf2}, we have applied an aggregate operator that computes the number of neighbors of the node \emph{country} (i.e. its degree), and the result has been stored as an attribute of such node.} 
\label{fig:transf3}
\end{figure} 
     
As introduced by Abiteboul and Vianu \cite{50376}, 
``database transformations map database instances to other database instances'', where such transformations include updates, queries, views and database restructuring.
Formally:

\begin{definition}(c.f. \cite{50398})
Let $S_1$ and $S_2$ two database schemas.
A \emph{transformation} from $S_1$ to $S_2$ is a recursively enumerable input-output relationship $T \subseteq inst(S_1) \times inst(S_2)$ which is invariant under every permutation of $\mathbf{U}$. 
\end{definition}


A CONTINUACION IRA LA DESCRIPCION DE LAS TRANSFORMACION SOPORTADAS POR LOS GRAPH QUERY LANGUAGES. 

G+ \cite{50285} is a graphical query language which introduced the notion of summary graph as a way of restructuring the results of a query.
Specifically, a G+ query is composed of two elements: 
a query graph which allows to express regular path queries; 
and a summary graph which specifies what to do with the results (i.e. subgraphs) of  matching the query graph against the database. 
The summary graph is restricted to have at most two nodes and one edge, labelled by constants and variables occurring in the query graph.

For instance, consider a graph database where nodes are labelled by the names of  people, and each directed edge is labelled with $M$ or $F$ to denote the relationship \emph{mother-of} or \emph{father-of} respectively.
Figure \ref{fig:Gplus} shows a G+ query which returns the pairs of people who share a common ancestor. 
Note that the summary graph $S$ allows to transform the subgraphs satisfying the query graph $Q$ into simple graphs representing the pairs of people with a common ancestor.   

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}

% rectangle 1
\draw[black] (1,1) rectangle (6,3.5);
\node[] (lr1) at (0.7,2.7) {Q:};

% nodo x
\node[circle,draw=black,inner sep=5pt] (n1) at (2,1.5) {$x$} ;

% nodo y
\node[circle,draw=black,inner sep=5pt] (n2) at (5,1.5) {$y$} ;

% nodo z
\node[circle,draw=black,inner sep=5pt] (n3) at (3.5,3) {$z$} ;

% edge e1
\draw[arrout,loosely dashed] 
(n3)[]to node (e1) {} (n1);
% edge label
\node[] (le1) at (2,2.5) {$(M \mid F)^{+}$};

% edge e2
\draw[arrout,loosely dashed] 
(n3)[]to node (e2) {} (n2);
% edge label
\node[] (le2) at (5,2.5) {$(M \mid F)^{+}$};

% rectangle 2
\draw[black] (7,1.3) rectangle (11,2.8);
\node[] (lr2) at (6.7,2.7) {S:};

% nodo n4
\node[circle,draw=black,inner sep=5pt] (n4) at (8,2) {$x$} ;

% nodo n5
\node[circle,draw=black,inner sep=5pt] (n5) at (10,2) {$y$} ;

% edge e3
\draw[arrout] 
(n4)[]to node (e3) {} (n5);

\end{tikzpicture}
\end{center}
\caption{Example of query in $G+$. The query is composed by the query graph $Q$ and the summary graph $S$. It returns the pairs of people ($x$,$y$) who share a common ancestor.} 
\label{fig:Gplus}
\end{figure} 


Additionally, G+ allows to express summary queries by allowing aggregate operators in the edge labels of the query graph. 
 There are two types of summary operators: path operators, which summarize on the values of the attributes along paths; and set operators, which summarize on the values of the attributes on a set of paths.
 For instance, Figure \ref{fig:Gplus2} shows a summarization query which is represented by an edge labelled with the summary operation $count,max$ where $count$ is the path operator and $max$ is the set operator. 
 In this case, the summary operation counts the number of edges in each path that connects $Peter$ with a descendant, and then calculates the maximum value. 
 Hence, the summary graph defines that the final output of the query is a list of nodes representing the most distance descendants of $Peter$.
 

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}

% rectangle 1
\draw[black] (1,1) rectangle (6,3);
\node[] (lr1) at (0.7,2.7) {Q:};

% nodo TO
\node[circle,draw=black,inner sep=3pt] (n1) at (2,2) {$Peter$} ;

% nodo X
\node[circle,draw=black,double,inner sep=9pt] (n2) at (5,2) {$x$} ;

% edge e1
\draw[arrout,loosely dashed] 
(n1)[]to node (e1) {} (n2);
% edge label
\node[] (le1) at (3.5,2.3) {$count,max$};

% rectangle 2
\draw[black] (7,1) rectangle (9,3);
\node[] (lr2) at (6.7,2.7) {S:};

% nodo X'
\node[circle,draw=black,inner sep=9pt] (n3) at (8,2) {$x$} ;

\end{tikzpicture}
\end{center}
\caption{Example of summarization query in G+. This query returns the most distance descendant(s) of $Peter$. } 
\label{fig:Gplus2}
\end{figure} 


GraphLog \cite{50209} is a variation of G+ where the summary graph was replaced by a distinguished edge in the query graph.
For instance, the query presented in Figure \ref{fig:Gplus} is expressed in  GraphLog as the single graph pattern shown in Figure \ref{fig:graphlog}.
In this case, the final result of the query is defined by the (distinguished) edge graphically represented by a bold line.
Note also that the distinguished edge is labelled with the literal $relative$ to define a new relationship between the pairs of people $(x,y)$ having a common ancestor $z$.

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}

% rectangle 1
\draw[black] (1,1) rectangle (6,3.5);
\node[] (lr1) at (0.7,2.7) {Q:};

% nodo x
\node[circle,draw=black,inner sep=5pt] (n1) at (2,1.5) {$x$} ;

% nodo y
\node[circle,draw=black,inner sep=5pt] (n2) at (5,1.5) {$y$} ;

% nodo z
\node[circle,draw=black,inner sep=5pt] (n3) at (3.5,3) {$z$} ;

% edge e1
\draw[arrout,loosely dashed] 
(n3)[]to node (e1) {} (n1);
% edge label
\node[] (le1) at (2,2.5) {$(M \mid F)^{+}$};

% edge e2
\draw[arrout,loosely dashed] 
(n3)[]to node (e2) {} (n2);
% edge label
\node[] (le2) at (5,2.5) {$(M \mid F)^{+}$};

% edge e3
\draw[arrout,fill=black,line width=0.5mm] 
(n1)[]to node (e3) {} (n2);
% edge label
\node[] (le3) at (3.4,1.3) {$relative$};

\end{tikzpicture}
\end{center}
\caption{Example of query in Graphlog.} 
\label{fig:graphlog}
\end{figure} 



GraphLog defines that the distinguished edge just can be labelled by a positive non-closure literal (i.e. it cannot contain a regular path expression).
However, the distinguished edge can be labelled with aggregate operators in order to express summarization queries.
For instance, assume a graph database where nodes represent cities and each edge is labelled with the distance between two cities.  
Figure \ref{fig:graphlog2} shows a GraphLog query which returns the shortest distance between two cities.
The query presents two main features: 
the regular expression $dist(\{D\})^{+}$ allows to compute the set of arbitrary paths between $Toronto$ and $Vancouver$; 
and the summarization expression $sdist(min(sum(D)))$ calculates the sum of the distances along each path, and then selects the minimum of such distances.

The expressive power of GraphLog with and without aggregates has been studied in \cite{50079} and \cite{50117} respectively.
In particular, the authors defined translations from GraphLog queries to Datalog programs, and studied fragments that can be computed efficiently. 
         
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}

% rectangle 1
\draw[black] (0,0) rectangle (7,5);
\node[] (lr1) at (0.7,2.7) {Q:};

% node 1
\node[circle,draw=black,inner sep=10pt] (n1) at (1.5,2.5) {} ;

% nodo 2
\node[circle,draw=black,inner sep=10pt] (n2) at (5.5,2.5) {} ;

% node3
\node[rectangle,draw=black,inner sep=3pt] (n3) at (1.5,0.5) {``Toronto''} ;

% node4
\node[rectangle,draw=black,inner sep=3pt] (n4) at (5.5,0.5) {``Vancouver''} ;

% edge e12
\draw[arrout,loosely dashed] 
(n1)[]to node (e12) {} (n2);
% edge label
\node[] (le12) at (3.6,3.5) {$sdist(min(sum(D)))$};

% edge e12b
\draw[arrout,line width=0.5mm,bend left=30] 
(n1)[]to node (e12b) {} (n2);
% edge label
\node[] (le12b) at (3.6,2.2) {$dist(\{D\})^{+}$};

% edge e13
\draw[arrout] 
(n1)[]to node (e13) {} (n3);
% edge label
\node[] (le13) at (2,1.5) {$name$};

% edge e24
\draw[arrout] 
(n2)[]to node (e24) {} (n4);
% edge label
\node[] (le1) at (6,1.5) {$name$};

%\draw[arrout,bend left=10] (n1) to 
%node[below, rectw] (e1) {} 
%(n2);

\end{tikzpicture}
\end{center}
\caption{Example of summarization query in GraphLog. This query returns the shortest distance between two cities. } 
\label{fig:graphlog2}
\end{figure} 

Levene and Poulovassilis studied notions of graph transformations in the context of hypernode data model. 
Recall that a hypernode is a graph whose nodes can encapsulate either a single values or a graph. 


\smallskip


Graph query languages that support data transformation:
\begin{itemize}
\item GOOD \cite{50076,50490} (1990)
\item The Hypernode Model and its Associated Query Language \cite{50167}(1990)
\item Concepts for Graph-Oriented Object Manipulation (GMOD) \cite{50114} (1992)
\item An Object-Oriented Pattern Matching Language (PaMaL) \cite{50269} (1993) 
\item GOAL, A Graph-Based Object and Association Language \cite{50082} (1993)
\item A Graph-Based Data Model and its Ramifications \cite{50152}(1995)
  define la noción de transformación
\item G-Log: A Graph-Based Query Language \cite{50081}(1995)
  tiene creación de objetos
\item Typing Graph-Manipulation Operations (GUL) \cite{50298} (2002)
\item Graphs-at-a-time \cite{90169} (2008)
  tiene un operator "composition" que permite generar graphs  
\item SNQL \cite{90697} (2011)
\item CONSTRUCT queries in SPARQL \cite{91294} (2015)
\end{itemize}


